SimMMDG: A Simple and Effective Framework for Multi-modal Domain Generalization

In real-world scenarios, achieving domain generalization (DG) presents significant challenges as models are required to generalize to unknown target distributions. Generalizing to unseen multi-modal distributions poses even greater difficulties due to the distinct properties exhibited by different modalities. To overcome the challenges of achieving domain generalization in multi-modal scenarios, we propose SimMMDG, a simple yet effective multi-modal DG framework. We argue that mapping features from different modalities into the same embedding space impedes model generalization. To address this, we propose splitting the features within each modality into modality-specific and modality-shared components. We employ supervised contrastive learning on the modality-shared features to ensure they possess joint properties and impose distance constraints on modality-specific features to promote diversity. In addition, we introduce a cross-modal translation module to regularize the learned features, which can also be used for missing-modality generalization. We demonstrate that our framework is theoretically well-supported and achieves strong performance in multi-modal DG on the EPIC-Kitchens dataset and the novel Human-Animal-Cartoon (HAC) dataset introduced in this paper. Our source code and HAC dataset are available at https://github.com/donghao51/SimMMDG.

==> tables/ablations.tex <==


\begin{table*}[t!]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
%& \multicolumn{4}{c}{\textbf{EPIC-Kitchen Activity Recognition Across Domains}}\\
%\cmidrule(lr){2-5}  %:)
CL & FS& DL & CT &  D2, D3 $\rightarrow$ D1 & D1, D3 $\rightarrow$ D2 & D1, D2 $\rightarrow$ D3  & \textit{Mean}\\
\midrule

& & &  & 55.86 & 56.27 & 54.21 & 55.45 \\
 $\checkmark$ & & &  & 52.18 & 64.80 & 62.22 &59.73  \\
 $\checkmark$ &  &  & $\checkmark$ & 51.49  & 67.07  &  63.24 &  60.60 \\
  $\checkmark$& $\checkmark$ & &  & 51.72 & 66.80 & 58.93 &  59.15\\
 $\checkmark$ & $\checkmark$ & $\checkmark$ &  & 55.17 & 64.00 & 64.37 & 61.18 \\
  $\checkmark$& $\checkmark$ &  $\checkmark$&   $\checkmark$& \textbf{57.93} & \textbf{68.67} & \textbf{66.32} & \textbf{64.31} \\
%\quad+ Translation Loss2 & \textbf{57.93} & \textbf{67.20} & \textbf{65.91} & \textbf{63.68} \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
%\vspace{-0.5em}
\caption{\textbf{Ablations} of each proposed module on EPIC-Kitchens dataset. 'CL' is supervised contrastive learning, 'FS' is feature splitting, 'DL' is distance loss, and 'CT' is cross-modal translation.}
%\vspace{-0.8em}
\label{tab:epic_kitchens_ab1}
\end{table*}



% \begin{table*}[t!]
% \centering
% \resizebox{0.8\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{lccccc}
% \toprule
% %& \multicolumn{4}{c}{\textbf{EPIC-Kitchen Activity Recognition Across Domains}}\\
% %\cmidrule(lr){2-5}  %:)
% \textbf{Method} & D2, D3 $\rightarrow$ D1 & D1, D3 $\rightarrow$ D2 & D1, D2 $\rightarrow$ D3  & \textit{Mean}\\
% \midrule

% Baseline  & 55.86 & 56.27 & 54.21 & 55.45 \\
% \quad+ Contrastive Learning  & 52.18 & 64.80 & 62.22 &59.73  \\
% \quad+ Split Embedding  & 51.72 & 66.80 & 58.93 &  59.15\\
% \quad+ Distance Loss & 55.17 & 64.00 & 64.37 & 61.18 \\
% \quad+ Translation Loss & \textbf{57.93} & \textbf{68.67} & \textbf{66.32} & \textbf{64.31} \\
% %\quad+ Translation Loss2 & \textbf{57.93} & \textbf{67.20} & \textbf{65.91} & \textbf{63.68} \\
% \bottomrule
% \end{tabular}

% \end{threeparttable}
% }
% \vspace{-0.5em}
% \caption{\textbf{Ablations} of each proposed module on EPIC-Kitchens dataset.}
% \vspace{-0.8em}
% \label{tab:epic_kitchens_ab1}
% \end{table*}



% \begin{table*}[t!]
% \centering
% \resizebox{0.65\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{lcccccc}
% \toprule
% %& \multicolumn{4}{c}{\textbf{EPIC-Kitchen Activity Recognition Across Domains}}\\
% %\cmidrule(lr){2-5}  %:)
% \textbf{Distance Type} & D2, D3 $\rightarrow$ D1 & D1, D3 $\rightarrow$ D2 & D1, D2 $\rightarrow$ D3  & \textit{Mean}\\
% \midrule


% %norm-2-norm  & 57.93 & 61.87 & 57.91 & 59.24 \\
% Cosine  & 53.56  &60.80  & 59.65 &  58.00\\
% $\ell_1$ norm &55.86  & 62.27 & 58.73 &58.95  \\
% $\ell_2$ norm & \textbf{57.93} & \textbf{68.67} & \textbf{66.32} & \textbf{64.31} \\
% \bottomrule
% \end{tabular}

% \end{threeparttable}
% }
% %\vspace{-0.5em}
% \caption{\textbf{Ablation} of different distance types in distance loss on EPIC-Kitchens dataset.}
% %\vspace{-0.8em}
% \label{tab:epic_kitchens_ab2}
% \end{table*}

==> tables/epic-ssdg.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{2}{c}{Source: D1}& \multicolumn{2}{c}{Source: D2}& \multicolumn{2}{c}{Source: D3}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  %:)
\textbf{Method} & D1$\rightarrow$ D2 & D1$\rightarrow$ D3 & D2 $\rightarrow$ D1 & D2 $\rightarrow$ D3& D3$\rightarrow$ D1& D3$\rightarrow$ D2  & \textit{Mean}\\
\midrule
%RSC (video-only)  & 50.34 & 45.98 &52.67 &58.80 &  42.71& 54.41 & 50.82 \\
%RSC (audio-only)  & 34.02 & 32.87 & 35.33& 43.33&40.45  & 42.09 &  38.02\\
DeepAll  &52.27& 51.75& 44.60& 54.11 & 48.05  & 56.67  &51.24  \\
MM-SADA~\cite{Munro_2020_CVPR}  &  50.67& 50.10&  51.49&  56.57   & 42.99      & 54.00       &  50.97 \\
RNA~\cite{Planamente_2022_WACV}  & 45.60& 46.30& 43.68 & 57.39& 49.66  & 55.87   &49.75\\
SimMMDG (ours) & \textbf{54.00} & \textbf{52.26}& \textbf{51.49} & \textbf{60.88}& \textbf{49.88}  & \textbf{60.53}  & \textbf{54.84} \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
%\vspace{-0.5em}
\caption{\textbf{Multi-modal single-source DG} on EPIC-Kitchens dataset using video and audio.}
%\vspace{-0.8em}
\label{tab:epic_ss}
\end{table*}





















% \begin{table*}[t!]
% \centering
% \resizebox{0.9\linewidth}{!}{
% \begin{threeparttable}
% \begin{tabular}{lcccccccc}
% \toprule
% & \multicolumn{2}{c}{Source: D1}& \multicolumn{2}{c}{Source: D2}& \multicolumn{2}{c}{Source: D3}\\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  %:)
% \textbf{Method} & D2$\rightarrow$ D1 & D3$\rightarrow$ D1 & D1 $\rightarrow$ D2 & D3 $\rightarrow$ D2& D1$\rightarrow$ D3& D2$\rightarrow$ D3  & \textit{Mean}\\
% \midrule
% %RSC (video-only)  & 50.34 & 45.98 &52.67 &58.80 &  42.71& 54.41 & 50.82 \\
% %RSC (audio-only)  & 34.02 & 32.87 & 35.33& 43.33&40.45  & 42.09 &  38.02\\
% DeepAll  & 44.60 & 48.05 &52.27 & 56.67& 51.75 & 54.11 &51.24  \\
% MM-SADA  &  51.49   & 42.99  &  50.67    & 54.00 & 50.10  &  56.57    &  50.97 \\
% RNA  & 43.68 & 49.66 & 45.60 & 55.87 & 46.30 & 57.39 &49.75\\
% SimMMDG (ours) & \textbf{51.49} & \textbf{49.88} & \textbf{54.00} & \textbf{60.53} & \textbf{52.26} & \textbf{60.88} & \textbf{54.84} \\
% \bottomrule
% \end{tabular}

% \end{threeparttable}
% }
% \vspace{-0.5em}
% \caption{\textbf{Multi-modal single-source DG} on EPIC-Kitchens dataset using video and audio.}
% %\vspace{-0.8em}
% \label{tab:epic_kitchens}
% \end{table*}

==> tables/hac-dg-more-modality.tex <==

\begin{table*}[t!]
\centering
\resizebox{0.7\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
%& \multicolumn{3}{c}{\textbf{Modality}} & \multicolumn{4}{c}{\textbf{EPIC-Kitchen Activity Recognition Across Domains}}\\
%\cmidrule(lr){2-4} \cmidrule(lr){5-8} %:)
\textbf{Method} & Video & Audio & Flow & A, C $\rightarrow$ H & H, C $\rightarrow$ A & H, A $\rightarrow$ C  & \textit{Mean}\\
\midrule

%RSC (flow-only) & & &$\checkmark$ & 55.17  & 63.33  &     59.65 &  59.38  \\
%Mixup (flow-only) & & &$\checkmark$ & 56.32   &  61.07 &   54.62   & 57.34   \\
DeepAll & $\checkmark$& $\checkmark$&  & 66.55  & 72.85  &  45.77 & 61.72 \\
MM-SADA~\cite{Munro_2020_CVPR} & $\checkmark$& $\checkmark$&  & 65.47  &  72.52 & 44.30  & 60.76 \\
RNA-Net~\cite{Planamente_2022_WACV} & $\checkmark$& $\checkmark$&   & 60.20  & 73.95  &  48.90 &  61.02\\
SimMMDG (ours)& $\checkmark$& $\checkmark$&  & 		\textbf{74.77} & \textbf{77.81} & \textbf{53.68} & \textbf{68.75} \\

\midrule
DeepAll & $\checkmark$& &$\checkmark$ & 76.78  &  70.64 &49.63 &  65.68 \\
MM-SADA~\cite{Munro_2020_CVPR} & $\checkmark$& &$\checkmark$ & 69.79 & 69.76  &49.45 & 63.00  \\
RNA-Net~\cite{Planamente_2022_WACV} & $\checkmark$& & $\checkmark$&  77.14 &74.94  &42.00 &  64.69 \\
SimMMDG (ours) & $\checkmark$& & $\checkmark$& \textbf{79.31} & \textbf{77.04} & \textbf{51.29} & \textbf{69.21} \\

\midrule
DeepAll & & $\checkmark$&$\checkmark$ & 50.04 &  59.71 &38.97 &  49.57 \\
MM-SADA~\cite{Munro_2020_CVPR} & &$\checkmark$ &$\checkmark$ & 46.58 & 61.81  &39.15 &  49.18 \\
RNA-Net~\cite{Planamente_2022_WACV} & & $\checkmark$&$\checkmark$ & 52.05 & 64.13  & 40.35&  52.18 \\
SimMMDG (ours) & & $\checkmark$&$\checkmark$ & \textbf{59.63} & \textbf{64.24} & \textbf{44.85} & \textbf{56.24} \\

\midrule
DeepAll & $\checkmark$& $\checkmark$& $\checkmark$ & 69.07&  71.30 &51.47 & 63.95  \\
MM-SADA~\cite{Munro_2020_CVPR} & $\checkmark$&$\checkmark$ &$\checkmark$ & 72.53 &  72.19 & 55.51&66.74   \\
RNA-Net~\cite{Planamente_2022_WACV} & $\checkmark$& $\checkmark$& $\checkmark$ &  69.00&  73.40 & 51.65& 64.68  \\
SimMMDG (ours) & $\checkmark$& $\checkmark$& $\checkmark$ & \textbf{77.65} & \textbf{79.03} & \textbf{56.62} & \textbf{71.10} \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
%\vspace{-0.5em}
\caption{\textbf{Multi-modal multi-source DG  with different modalities} on HAC dataset.}
%\vspace{-0.8em}
\label{tab:hac-dg2}
\end{table*}

==> tables/hac-dg.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.6\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccccc}
\toprule
%& \multicolumn{4}{c}{\textbf{HAC Dataset Activity Recognition Across Domains}}\\
%\cmidrule(lr){2-5}  %:)
\textbf{Method} & A, C $\rightarrow$ H & H, C $\rightarrow$ A & H, A $\rightarrow$ C  & \textit{Mean}\\
\midrule
%RSC (video-only)   &   &   &   &  \\
%RSC (audio-only)   &   &   &   &  \\
DeepAll  & 66.55  & 72.85  &  45.77 & 61.72 \\
MM-SADA   & 65.47  &  72.52 & 44.30  & 60.76 \\
RNA-Net~\cite{Planamente_2022_WACV}   & 60.20  & 76.16  &  48.90 &  61.75\\
SimMMDG (ours) & 		\textbf{72.82} & \textbf{77.70} & \textbf{54.04} & \textbf{68.19} \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
\vspace{-0.5em}
\caption{\textbf{Multi-modal multi-source DG} on HAC dataset using video and audio.}
%\vspace{-0.8em}
\label{tab:hac-dg}
\end{table*}

==> tables/hac-ssdg.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.6\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{2}{c}{Source: H}& \multicolumn{2}{c}{Source: A}& \multicolumn{2}{c}{Source: C}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  %:)
\textbf{Method} & H$\rightarrow$ A & H$\rightarrow$ C & A $\rightarrow$ H & A $\rightarrow$ C& C$\rightarrow$ H& C$\rightarrow$ A  & \textit{Mean}\\
\midrule
DeepAll  &66.11 & 43.01 &63.45 & 37.68 &  46.86 & 58.94  &  52.68\\
MM-SADA~\cite{Munro_2020_CVPR}  &65.89 & 37.22&57.75 & 40.90 &  49.82 & 62.91  & 52.42 \\
RNA~\cite{Planamente_2022_WACV}   & 65.67& 42.92& 61.72& 38.69 & 47.66  & 61.59  &  53.04\\
SimMMDG (ours) & \textbf{66.67} & \textbf{44.21}& \textbf{68.42} & \textbf{46.05}& \textbf{54.43}  & \textbf{72.73}  & \textbf{58.75} \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
%\vspace{-0.5em}
\caption{\textbf{Multi-modal single-source DG} on HAC dataset using video and audio.}
%\vspace{-0.8em}
\label{tab:hac_ss}
\end{table*}

==> tables/single-modal-DG-rebu.tex <==
\begin{table}[h!]

\begin{adjustbox}{width=0.6\linewidth}
\begin{tabular}{lcccc}
\toprule
%Method & \makecell[c]{D2, D3 \\ $\rightarrow$ D1} & \makecell[c]{D1, D3 \\ $\rightarrow$ D2} & \makecell[c]{D1, D2 \\ $\rightarrow$ D3}  & \textit{Mean}\\
\textbf{Method} &D2, D3 $\rightarrow$ D1 & D1, D3 $\rightarrow$ D2 & D1, D2 $\rightarrow$ D3  & \textit{Mean}\\
 \noalign{\smallskip} \hline \noalign{\smallskip}
RSC (V) & 50.11 & 62.53 & 58.73& 57.12\\    
RSC (A) & 36.55 & 43.73 & 48.15& 42.81\\ 
RSC (F) & 55.17 &63.33  &59.65 & 59.38\\ 
Mixup (V) & 49.20 & 59.73 &59.96 &56.30\\ 
Mixup (A) & 35.17 &  40.80&45.07 & 40.35\\ 
Mixup (F) &56.32  & 65.60 & 54.62&58.85\\  
Fishr (V) & 53.79 & 63.47 & 61.09 & 59.45 \\ 
Fishr (A) & 37.47 & 44.80 & 47.43 & 43.23 \\ 
Fishr (F) & 54.25 & 63.87 & 59.14 & 59.09 \\ 


\hline \noalign{\smallskip}

\makecell[c]{SimMMDG \\(V+A+F)} & \textbf{63.68} & \textbf{70.13} & \textbf{67.76} & \textbf{67.19} \\ 
\bottomrule
\end{tabular}
\end{adjustbox}

%\vspace{+0.05cm}
%\caption{Comparison with single-modal DG methods on EPIC-Kitchens dataset. V: video, A: audio, F: optical flow.}
%\vspace{-1cm}

\label{tab:single-re}
\end{table}



